Dark matter search in a Beam-Dump eXperiment (BDX) at Jefferson Lab

MeV-GeV dark matter (DM) is theoretically well motivated but remarkably unexplored. This proposal presents the MeV-GeV DM discovery potential for a $\sim$1 m$^3$ segmented CsI(Tl) scintillator detector placed downstream of the Hall A beam-dump at Jefferson Lab, receiving up to 10$^{22}$ electrons-on-target (EOT) in 285 days. This experiment (Beam-Dump eXperiment or BDX) would be sensitive to elastic DM-electron and to inelastic DM scattering at the level of 10 counts per year, reaching the limit of the neutrino irreducible background. The distinct signature of a DM interaction will be an electromagnetic shower of few hundreds of MeV, together with a reduced activity in the surrounding active veto counters. A detailed description of the DM particle $\chi$ production in the dump and subsequent interaction in the detector has been performed by means of Monte Carlo simulations. Different approaches have been used to evaluate the expected backgrounds: the cosmogenic background has been extrapolated from the results obtained with a prototype detector running at INFN-LNS (Italy), while the beam-related background has been evaluated by GEANT4 Monte Carlo simulations. The proposed experiment will be sensitive to large regions of DM parameter space, exceeding the discovery potential of existing and planned experiments in the MeV-GeV DM mass range by up to two orders of magnitude.

==> Makefile <==
#
# Makefile to latex document, uncompress .ps files etc...
# original version : Mark Ito
# modified:
#
#     BDX-proposal_main  - Elton Smith 03/22/16   -- use pdflatex
#
#
TEX_FILES_0 = BDX-proposal_main BDX-proposal_intro BDX-proposal_motivation BDX-proposal_measurement \
              BDX-proposal_setup BDX-proposal_results BDX-proposal_summary BDX-proposal_BDXprototype BDX-proposal_Drift cormorino_appdx newcomm \
              BDX-proposal_phenomenology
TEX_FILES = $(addsuffix .tex,$(TEX_FILES_0)) # add .tex suffix

PNG_FILES_0 = figs/snowmass
PNG_FILES = $(addsuffix .png,$(PNG_FILES_0)) # add .ps suffix

PDF_FILES_0 = figs/fig2 figs/ElectronRecoilSpectrum_Mchi10_mA50 figs/ElectronRecoilSpectrum_Mchi68_mA150 \
              figs/fig1 figs/exp_setup figs/BDXvsE137mchi10_Nucleon_Erec1MeV figs/BDXvsE137mchi10_Nucleon_Erec1MeV \
              figs/BDXvsE137mchi10delta50 figs/cormorino figs/signal figs/cormorino_veto figs/halld_beamdump \
              figs/det1 figs/det2 figs/det4 figs/kine1 figs/kine3 figs/kine4 figs/kine5 figs/E_nu figs/neutrino \
              figs/cosmics figs/BDXvsE137mchi10_Electrons_VariousThresholds
PDF_FILES = $(addsuffix .pdf,$(PDF_FILES_0)) # add .pdf suffix

C_FILES_0 = 
C_FILES = $(addsuffix .C,$(C_FILES_0)) # add .C suffix


all : BDX-proposal_main.pdf

BDX-proposal_main.pdf : $(TEX_FILES) Makefile BDX-proposal_main.bbl $(PDF_FILES) \
               $(PNG_FILES)                # make the pdf file
	pdflatex BDX-proposal_main.tex
	pdflatex BDX-proposal_main.tex

BDX-proposal_main.bbl : BDX-proposal_main.bib $(TEX_FILES) $(PS_FILES) $(EPS_FILES)
	pdflatex BDX-proposal_main
	bibtex BDX-proposal_main

tar : $(TEX_FILES) $(PS_FILES) $(EPS_FILES) # tar files; will remove old tar files
	rm -f BDX-proposal_main.tar
	rm -f BDX-proposal_main.tar.gz
	rm -rf BDX-proposal_main
	mkdir BDX-proposal_main
	mkdir BDX-proposal_main/figs
#	cp BDX-proposal_main.ps BDX-proposal_main
	cp BDX-proposal_main.bib BDX-proposal_main
	cp $(TEX_FILES) BDX-proposal_main
#	cp $(EPS_FILES) BDX-proposal_main
	cp $(PNG_FILES) BDX-proposal_main/figs
	cp $(PDF_FILES) BDX-proposal_main/figs
#	cp $(C_FILES) BDX-proposal_main
	cp BDX-proposal_main.pdf BDX-proposal_main
	cp Makefile BDX-proposal_main
	tar cvf BDX-proposal_main.tar BDX-proposal_main
	gzip BDX-proposal_main.tar
#	rm -rf BDX-proposal_main

%.ps : %.dvi
	dvips -t letter -o $*.ps $* 
	dvipdf $*.dvi $*.pdf


%.dvi : %.tex
	latex $*
	latex $*

%.pdf : %.tex
	pdflatex $*
	pdflatex $*

%.ps : %.ps.gz
	gunzip -l $*.ps.gz
	rm -f $*.ps
	gunzip -c $*.ps.gz > $*.ps

%.eps : %.eps.gz
	gunzip -l $*.eps.gz
	rm -f $*.eps
	gunzip -c $*.eps.gz > $*.eps

#
#
% : %.dvi
#	'rm' -rf $*
#	latex2html $*      # produce html pages

clean:
	rm -f HallD_ESAD.dvi BDX-proposal_main.ps




==> cormorino_appdx.tex <==
\begin{figure}[t!] 
\center
\includegraphics[width=12cm]{figs/cormorino.pdf}
 \caption{ (Left) CAD representation of the CORMORINO detector, made by 9 bars of plastic scintillators read by 3PMTs, each read on both sides by a a 3'' PMTs . (Right) A picture of the detector mounted on its support and cabled.
 }\label{fig:cormorino}
\end{figure}

\begin{figure}[t!] 
\center
\includegraphics[width=14cm]{figs/signal.pdf} 
 \caption{Left: a typical signal from CORMORINO and its digitization. Right: time resolution of CORMORINO measured with cosmic muons. }\label{fig:signal}
\end{figure}
\section{A study case: CORMORINO and JLab Hall-D beam-dump}  
In this Section we report results of a study  for a possible beam-dump experiment at JLab.
The case study places an existing detector, CORMORINO, downstream of the Hall-D beam-dump, as shown in 
Fig.~\ref{fig:exp_setup}. 
We study this option in detail because CORMORINO  implements a technology that we consider as a viable option for a full scale experiment 
and that,  with  minor modifications, can be easily used to measure   cosmogenic backgrounds and validate simulations.
Beam-related backgrounds were simulated in the Hall-D beam-dump configuration because, being above ground, this represents
 a set-up where  CORMORINO could be easily installed  with no need for major civil construction to perform a test run and validate the MC estimates. 
Based on these considerations, in this Section we report estimates for beam-related and beam-unrelated background rates in this experimental configuration as well as the expected signal rates. 
These results will be used to estimate the counts expected in a full experiment whose 
concept,  including a $\sim $1 m$^3$ optimised detector placed behind a high intensity Hall beam-dump (A or C), is  discussed  in the next section.

\begin{figure}[t!] 
\center
\includegraphics[width=14cm]{figs/cormorino_veto.pdf} 
 \caption{The veto detector sourrrounding CORMORINO is made by sheets of 2 cm thick plastic scintilators coupled to PMTs by shaped Plexiglas light guides. A thin layer of lead shields gamma's produced by particles decaying between the veto and CORMORINO. The detector is currently being assembled.} \label{fig:cormorino_veto}
\end{figure}


\subsection{The CORMORINO detector}
The CORMORINO detector is a 0.036 m$^3$ cube made of plastic scintillator bars read by PMTs. 
It is a prototype built for the experiment CORMORAD (COre Reactor MOnitoRing by an Antineutrino Detector), aiming to use antineutrino to monitor power and isotopic composition of the core of a commercial nuclear power plant. The 1.5 - 10 MeV antineutrinos  produced by the fragment of the  nuclear fission interact with protons of plastic scintillator by inverse beta decay producing a positron and a neutron. The plastic scintillator, acting as an active target, provides a high number of protons and a good detection capability for both the positron ionization and neutron capture. The detector is made by nine optical channels, each consisting  of four 5x5x30 cm$^3$ plastic scintillator bars  (NE102) individually wrapped in aluminised Mylar.  The four bars are coupled on each side to a  Photonis XP2312 3''  photomultiplier via a 10x10x5 cm$^3$ scintillator block,  acting as light guide. Figure~\ref{fig:cormorino} shows a CAD drawing and a picture of the detector. The 9 (Left) +  9 (Right) PMTs are connected to 250 MHz 16ch JLab fADC boards for signal digitisation.
A typical signal is shown  on the left panel  of Fig.~\ref{fig:signal}. In the same Figure on the right,   the time resolution measured with cosmic muons is shown. With the current PMT gain, an energy deposition in the plastic scintillator  of 1 MeV corresponds to a signal of 8 mV in amplitude in each PMT. In spite of the aged  plastic scintillator used in CORMORINO, the measured time resolution for MIPs is $\sigma_T \sim 110$ ps.
With new plastic, better optical coupling and optimised PMTs a time resolution of $\sim 50$ ps  can be easily obtained as demonstrated by the new CTOF detectors built for CLAS12~\cite{Baturin:2005hr}. 
The low rate expected in the experiment does not require a selective trigger and therefore the DAQ scheme that is  implemented
uses a simple L$\&$R single-bar coincidence to save the full wave shape stored in the fADC. The trigger threshold can be set at 5 mV (corresponding to the energy deposited by a  600 keV electron) leaving to the off-line analysis more sophisticated selections for background suppression\footnote{In fact, having the full shape for each sample it is possible to do some particle identification, time measurement and time correlation between samples to reject neutron capture, rare muon decays, etc. }. We are currently building a hermetic charged-particle veto counter based on 2 cm thick plastic scintillator planes to be placed  in front of each of the 6 faces of the CORMORINO to reject cosmic muons and further reduce backgrounds. A layer of 5 cm of lead between the veto and the detector surface will shield from low energy gamma
 from particles decaying inside the external iron shield. Figure~\ref{fig:cormorino_veto}  shows the layout of the active and passive veto surrounding CORMORINO. 


\subsection{The Hall-D beam-dump}
The Hall-D at JLab is expected to receive from CEBAF a 12 GeV electron beam with an average current of  $\sim$200 nA.
This moderate current  is not  the optimal choice for a full scale  experiment at JLab but the simplified logistic encouraged us to study this configuration in case beam-related backgrounds were found to be dominant, calling for a test run.
The beam line delivering electrons to Hall-D runs above the ground in the last section of its path, in proximity of the beam-dump. This simplifies any possible detector deployments behind the beam-dump enclosure with access from all sides. To set up the experiment  a hut hosting the detector in a water-tight and air-conditioned environment with few services such as power and network connection is required. For this option a shield for cosmogenic neutrons and cosmic rays need to be artificially implemented, providing a pit of few meters of iron all around the detector. %\footnote{Digging a hole in the ground behind the Hall-A beam-dump would result in a under-ground naturally shielded environment.}

The Hall-D beam-dump is made by an aluminum cylinder, $\sim$25 cm in diameter and $\sim$100 cm in length, followed by a  $\sim$30 cm long copper cylinder of the same diameter. They are both cooled by circulating water. The full drawing of the beam-dump is shown in the left panel of  Fig.~\ref{fig:halld_bd}. The beam-dump is housed in a concrete ($\sim$0.8 m thick) and iron ($\sim$4 m thick) enclosure shown in the right panel of the same figure.
To further reduce  possible radiations, another shield made by  $\sim$8 m of iron has been added downstream.
\begin{figure}[t!] 
\center
\includegraphics[width=16.5cm]{figs/halld_beamdump.pdf}  
 \caption{ (Left) The Hall-D beam-dump;  the aluminum and copper cylinder where the beam stops and the cooling pipes surrounding the dump are clearly visible. (Right) The beam-dump enclosure:  only the external concrete wall is visible while the iron shield is hidden inside. }\label{fig:halld_bd}
\end{figure} 



\subsection{Simulations of the  experimental set-up}\label{sec:expsetup}
Both the CORMORINO detector and the Hall-D beam-dump geometry have been implemented in GEANT4 within the GEMC simulation package~\cite{gemc}. In the following sections we 
present some results concerning the beam-related background, the cosmogenic background and the expected rates from an elastic interaction of a $\chi$ particle.  The $\chi$ signal was simulated assuming the dominance of elastic DM interaction as discussed in Sec.~\ref{sec:elastic}.
Figure~\ref{fig:cormorino_gemc} shows the detector as implemented in the simulations. As already mentioned
CORMORINO is positioned $\sim$15 m downstream the beam-dump, surrounded by a 1 meter of iron acting as a passive shield for cosmic neutrons and gammas. 
\begin{figure}[t!] 
\center
%\includegraphics[width=14cm]{figs/cormorino_gemc.pdf} 
\includegraphics[width=0.4\textwidth]{figs/det1.pdf} 
\includegraphics[width=0.285\textwidth]{figs/det2.pdf}
\includegraphics[width=0.285\textwidth]{figs/det4.pdf}

 \caption{Implementation of the CORMORINO detector in GEMC. The section on the right shows the 9 optical channels (each made by 4 plastic scintillator bars), with a cylinder surrounding the detector acting as an active veto. In the middle plot, the lead shielding (in green) is shown. The  section on the left shows the detector and veto inside a 1 m thick iron pit to reduce cosmogenic background.   }\label{fig:cormorino_gemc} 
\end{figure}
 

\begin{table}[htp]
\caption{Relevant parameters of the theory for the two scenarios. The resulting number of $\chi$ produced per electron on target  (EOT) and the elastic interaction cross section $\sigma_{\chi-p}$ are also reported.}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
 & S.I &  S.II\\
\hline\hline
 M$_\chi$ & 10 MeV &  68 MeV\\
 \hline
M$_{A^\prime}$ & 50 MeV  & 150 MeV\\
\hline
$\epsilon$ & 10$^{-3}$ &10$^{-3}$\\
\hline
$\alpha_{Dark}$ & 0.1  & 0.1\\ 
\hline\hline
N$_\chi$ pairs produced per EOT& 3.4 10$^{-10}$ &3.4 10$^{-11}$  \\
\hline
$\sigma_{\chi-p}$ & 1.4 nb  &  0.14 nb\\
\hline\hline
\end{tabular}
\end{center}
\label{tab:twoscen}
\end{table}%

\subsubsection{$\chi$ production and  $\chi$-p elastic scattering in CORMORINO}
Detection of a $\chi$ particle in CORMORINO involves two steps: the A$^\prime$ electro-production and subsequent decay  A$^\prime \to \chi \bar\chi$, happening in the very first layer of the beam-dump,  and the elastic scattering of a $\chi$ on a proton of the detector.   Both processes depend on four
parameters: the mass of the $\chi$ (M$_\chi$), the mass of the exchanged A$^\prime$ (M$_{A^\prime}$), the coupling constant between the electron and the A$^\prime$
($\epsilon$) and the coupling constant between the $\chi$ and the A$^\prime$ ($\alpha_{Dark}$).  
We explored two possible scenarios, S.I and S.II, for which the corresponding parameters are  reported in Tab.~\ref{tab:twoscen}. The table also reports the resulting $\chi$ production rate (per EOT or {\it Electron On Target}) and the corresponding elastic cross section on a proton in the detector.
Figure~\ref{fig:kinea} shows the kinematics of the $\chi$ within the CORMORINO acceptance, assuming a 12 GeV electron beam (left and right plots correspond to S.I and S.II respectively). 
\begin{figure}[t!] 
\center
\includegraphics[width=16cm]{figs/kine1.pdf}  
\includegraphics[width=16cm]{figs/kine3.pdf}  
\caption{Top: the kinetic energy of  the $\chi$ particle  produced by 12 GeV electron beamin the two scenarios studied (left S.I, right S.II). 
Bottom: the distribution of $\chi$ events hitting the CORMORINO surface (left S.I, right S.II).}
\label{fig:kinea}
\end{figure} 
Figure~\ref{fig:kinec} shows the energy deposited in the detector by the  proton recoils  induced by the $\chi$-p elastic scattering. 
The red histogram shows the deposited energy while the black shows the reconstructed energy for the proton detection, including  the light quenching effect in the scintillator.
It is worth noticing that a sizeable fraction of events deposits a visible energy greater than 1 MeV.
%\begin{figure}[t!] 
%\center
%\includegraphics[width=12cm]{figs/kine4.pdf} 
 %\caption{Energy deposited in the detector by a the struck proton after a $\chi$-p eleastic scattering  (left S.I, right S.II). }\label{fig:kineb}
%\end{figure} 
To evaluate the number of  detected events in CORMORINO, we required a single hit defined as the coincidence of the PMTs coupled to the same scintillation bar.
For both scenarios we evaluate the rates for two thresholds: 1 MeV and 10 MeV\footnote{To realistically simulate threshold effects, we applied a threshold to each PMT, independently.}.
%Being the CORMORINO scintillating bar limited to 40cm in length, the attenuation of the light in plastic, included in the simulations, provides a negligible effect.\footnote{The plastic scintillator used in CORMORINO is an %old sample of NE110 dating back to 30 years ago. The measured attenuation lenght is about 110cm and therefore its effect on a 40cm bar is negligible. This is even more true for a standard new plastic scintillator bar of the same size being the attenuation lenght  in the range of 200-250 cm.}
The effect of light attenuation in the scintillator was also included in the simulations, even if the effect is known to be small give the size of the detector.
\begin{figure}[t!] 
\center
\includegraphics[width=16.5cm]{figs/kine5.pdf} 
 \caption{The energy deposited (red) and reconstructed (black) in CORMORINO. The recontructed energy spectrum includes the effect of light quenching in the two scenarios (left S.I, right S.II). }\label{fig:kinec}
\end{figure} 
The expected $\chi$-p elastic detection rate (per $\mu$A)   for a  threshold of 1 MeV (10 MeV) is therefore:
\be
R_{elastic \;\chi}^{S.I}=   1.0\; 10^{-5} {\rm Hz}/ \mu {\rm A} \;\; (1.2 \;10^{-6} {\rm Hz}/\mu {\rm A})
\ee
\be
R_{elastic \;\chi}^{S.II}=   2.0\; 10^{-7} {\rm Hz}/\mu {\rm A} \;\; (0.7 \;10^{-7} {\rm Hz}/\mu {\rm A})
\ee


\subsubsection{Beam-related background}
The beam-related background has been simulated generating 1.6 10$^9$ 12 GeV EOT impinging on the beam-dump, corresponding  to 1.2 ms of 200 nA beam.
The only particles exiting from the beam-dump and crossing the detector area are $\nu$
 and $\bar\nu$ from the $\pi^+$ decay
 ($\pi^+ \to \mu^+ \nu_\mu$) and the $\mu^+$ decay ($\mu^+ \to e^+ \bar\nu_\mu \nu_e$) 
with a ratio of about 1.1 $\nu_\mu$ : 1 $\nu_{\bar\mu}$ : 1.1 $\nu_e$. 
 Negative pions are captured by nuclei before they can decay and therefore do not contribute to the neutrino counting. The energy spectrum of the 3 species is reported on the left panel of 
Fig.~\ref{fig:E_nu}: the positive pion decays at rest providing a monocromatic set of $\nu_\mu$ of 33.9 MeV (M$_\pi$-M$_\mu$). Neutrinos from $\mu^+$ decay share a total energy of 105.1 MeV (M$_\mu$-M$_e$), which results in a upper limit for the energy of the  $\nu_{\bar\mu}$ and  $\nu_e$.  These neutrinos origins inside the beam-dump as shown in the right panel of Fig.~\ref{fig:E_nu}. 
The rates of neutrinos  crossing the detector area, approximately equal for the three species, are $\sim$7.5 10$^6$ Hz/$\mu$A while the integrated rate is  $\sim$2.2 10$^7$ Hz/$\mu$A.
Neutrinos with energy in the range 2-100 MeV mainly interact by CC interaction  ($\bar\nu p \to e^+$ n) with a cross section of about  $\sigma_{\bar\nu p}\sim10^{-40}$ cm$^2$.
Considering  the volume of CORMORINO and assuming a detection efficiency of $\epsilon_{e^+ detection}=50\%$ with 1 MeV threshold (5$\%$ for 10 MeV
threshold), the background rate   is given by:
\be
R_{B-rel}^{\nu} = R^{\nu} \;\sigma_{\bar\nu p}\; N_{Avogadro} 1/A \; \rho_{plastic} \; L_{CORMORINO} \; \epsilon_{e^+ detection}= 2\;10^{-9} {\rm Hz}/\mu  {\rm A} \;\;(2\;10^{-10}  {\rm Hz}/\mu {\rm A})
\ee
No neutrons or other particles are observed within the  generated statistics. This allows us to set only an upper limit on the corresponding rate that we will improve by increasing the Monte Carlo statistics. 

Beside the beam-related background estimated by MC simulations, in Sec.~\ref{sec:systematics} we discuss  additional  checks that could be performed during the run by changing the experimental set-up (e.g. off-axis and  on/off  measurement, noise on PMTs, .etc.) to determine systematic  effects that  we may have under-evaluated or neglected by MC simulations.
\begin{figure}[t!] 
\center
\includegraphics[width=17cm]{figs/E_nu.pdf}  
 \caption{Left: the energy spectrum of beam-related neutrinos crossing CORMORINO surface  (black: total spectrum; red: $\nu_\mu$, green: $\bar \nu_\mu$,  blue: $\nu_e$). Right: the vertex of the decaying primary particles ($\mu$ and $\pi$) starting at the beam-dump location and extending for 1 m downstream. }\label{fig:E_nu}
\end{figure} 



\subsubsection{Beam-unrelated background}
Beam-unrelated background is mainly due to cosmic neutrons, cosmic muons and their decay products, including  rare decays of muons producing gamma's between the passive shield and the active veto. In this Section we briefly present ideas on how to reduce these backgrounds, that could be applicable to  a new, full-scale, optimized detector.
We will also present some preliminary results of MC simulations specifically for the CORMORINO set-up. To validate  MC simulations and optimize the selection algorithms,
we are planning to perform an extensive campaign of measurements with the CORMORINO detector in the same experimental conditions of a real experiment (detector placed  above the ground, same shielding as reported here, etc).


\paragraph{Time-Correlation}
Beam-uncorrelated background can be rejected by requiring a time coincidence between the RF signal and the event recorded by the detector. Even if the studied case of a plastic scintillator detector provides a sub-ns response to a $\chi$ scattering, the almost-CW structure of the CEBAF beam does not allow to take full  advantage of this technique. In fact the bunch separation expected with the 12 GeV operations is $\Delta$T=4.0 ns to be compared with the measured time  resolution of CORMORAD of $\sigma_T\sim$200 ps for 1 MeV deposited energy. The background reduction factor, $R$, can be expressed as the ratio between the time coincidence window width (3$\sigma_T$)  and $\Delta$T providing for JLab-CORMORINO(-like) conditions:
\be
R=\frac{3 \sigma_T}{\Delta T}\sim 20\% 
\ee
It is worth to notice that  for  the set up discussed in this paper, a detector placed 15 m away from the beam-dump, $\chi$ masses between 0 - 500 MeV result in a time-of-flight  spread below  $\sigma_T$=200 ps (0 - 170 MeV for $\sigma_T$=20ps).
The same argument applies to the $\chi$ momentum spread: any  p$_\chi$ between 6 GeV and 100 MeV correspond to a time-of-flight spread below  $\sigma_T$=200ps (6 GeV -  350 MeV for $\sigma_T$=20ps). This rational suggests that,  for a fast detector ($\sigma_T\sim$70-100ps) the rejection factor for uncorrelated background can be reduced up to a factor of ten. This will be further discussed in in Sec.~\ref{sec:r-and-d}. In the following, we are not considering the timing cuts and therefore the background rejection factor needs to be added to the obtained results.


\paragraph{Directionality} 
Beside time-correlation, directionality could help in reducing the cosmogenic background. In fact the angular distributions of  cosmic muons 
(and their decay products)  and cosmic neutrons are peaked around the vertical (the angular distributions are proportional to $\cos^2{\theta}$ and   $\cos^3{\theta}$ respectively) while 
the $\chi$s are expected to follow the beam direction. The simple detector described here (a plastic scintillator cube) 
%  : does
does not provide directionality capability for a single-hit interactions  but this considerations can be used in designing a full-scale, optimized detector as report in Sec~\ref{sec:r-and-d}.\\

In the following we report  rate estimates for all species of cosmogenic background as obtained by GEANT4 simulations.


\begin{figure}[t!] 
\center
\includegraphics[width=16cm]{figs/neutrino.pdf} 
 \caption{Cosmic neutrino flux and interaction cross section. }\label{fig:neutrino}
\end{figure} 
\paragraph{Cosmic neutrinos}  
Cosmic neutrinos interactions represent a negligible contribution to the uncorrelated background. The only sizeable fluxwe need to consider is for solar neutrinos ~\cite{Bahcall:2004fg} with energy below 10 MeV (see Fig.~\ref{fig:neutrino}-Left)  a rate on CORMORINO of $R^{Cosmic \nu}_{E_\nu<10 MeV}\sim 3 \;10^{11}$ Hz.  Low energy neutrinos (E$_\nu<$10 MeV)
%  : interact
 interact with protons in the  detector mainly by inverse beta decay ($\bar\nu p \to e^+$ n), producing a positron that carries almost all the neutrino energy and could mimic a $\chi$ interaction. The corresponding cross section~\cite{GilBotella:2004bv},  reported in Fig.~\ref{fig:neutrino}-Right) is in the range of  $\sigma_{\bar\nu p}\sim 3\; 10^{-42}$ cm$^2$.
The background rate,  considering  the volume of CORMORINO and assuming a detection efficiency of $\epsilon_{e^+ detection}=50\%$ 
 with 1 MeV thresholds (and 5$\%$ for 10 MeV threshold),  is given by:
\be
R_{Bg}^{\nu} = R^{Cosmic \nu}_{E_\nu<10 MeV} \;\sigma_{\bar\nu p}\; 1/A N_{Avogadro} \; \rho_{plastic} \; L_{CORMORINO} \; \epsilon_{e^+ detection}= 10^{-6}  {\rm Hz}\;\;  (10^{-7} {\rm Hz} )
\ee
The flux of cosmic neutrino
with higher energy is several orders of magnitude smaller, which does not compensate for the increase in the interaction cross section. Moreover, the elastic scattering  on a proton transfers a small amount of energy reducing the probability of detecting the struck proton. For all these reasons the cosmic neutrino background is negligible with respect to the other sources.
\begin{figure}[t!] 
\center
\includegraphics[width=16cm]{figs/cosmics.pdf} 
 \caption{Flux of cosmic neutron (left) and muons (right). }
 \label{fig:cosmic} 
\end{figure} 
 
\paragraph{Cosmic neutrons}
A cosmic neutron interacting with CORMORINO can produce a signal over the trigger threshold identical to a  $\chi$ hit. 
Considering the typical interaction length of neutrons in plastic, the 2 cm thick active veto has a small chance to detect the incoming neutrons. On the other hand, the veto is  sometimes useful to reject  neutron events producing  hadronic showers  in  the heavy passive shielding when some charged fragments reach the detector.
 To estimate the rate of single hits in CORMORINO (mimicking a $\chi$ interaction), we generated a realistic
cosmic neutron flux as reported in Fig.~\ref{fig:cosmic}-Left with the  parametrization from Ref.~\cite{1369506,1589260}.
The overall neutron rate in open-air at  sea level (integrating over all energies and angles) is $\sim$64 Hz/m$^2$, (corresponding to a differential flux of  $\sim$50 Hz/m$^2sr$).
The CORMORINO neutron detection efficiency $\epsilon_{n \; cosmic}$ depends on  the surrounding shielding, the incoming neutron energy ($E_n$) and  the detection threshold ($E_{Thr}$).  
%  : epsilon non e' 0, ma circa 4E-5 a 1 MeV e 9E-6 a 10 MeV. Metti ~ 0 per dire che sono molto piccole?
Considering the 1 m  iron shield,  and a detection threshold of 1 MeV  (10 MeV) we found that  the detector is blind ($\epsilon_{n \; cosmic}\sim0$) for neutrons with energy lower than 50 MeV (100 MeV). 

Thus, the overall visible  rate for a detection threshold of 1 MeV (10 MeV) is:
\be
R_{Bg}^n=   2.7\; 10^{-3} {\rm Hz} \; \; (0.6\; 10^{-3} {\rm Hz} )
\ee

\paragraph{Cosmic muons}
Cosmic muons are by far the main source of uncorrelated background  in a plastic scintillator detector. Fortunately, the most part of muons interacts with the veto counter and CORMORINO  releasing the typical energy of a MIP, that can be tracked and rejected exploiting the detector segmentation. Another source of background is due  to muons decaying within the detector and between the shielding and the veto counter. In the following we report rate estimates based on MC simulations for  the measured muon flux shown in Fig.~\ref{fig:cosmic}-Right from Ref.~\cite{Appleton:1971kz}.

\subparagraph{Crossing muons}  
The combination of the active veto,  also sensitive to   cosmic muons crossing at large angles,  together with the CORMORINO identification capability (segmentation) sizeably  reduces the number of crossing muons. 
The cosmic muon flux rate on the CORMORINO surfaces,  is 30.3 Hz (40$\%$  hits the top face and the remaining 60$\%$ hits the lateral sides) neglecting the  shielding.
The effect of 1 m iron shielding and 5 cm thick lead is to suppress   muons with momentum  $<$1.45 GeV/c, reducing the flux on the detector to R$^{All\;\mu}\sim$ 4.5 Hz, and 4 Hz (3.9 Hz) for hits   over a 1 MeV (10 MeV) threshold in CORMORINO.
Crossing muons usually provides 2 hits on the veto detector and  $\ge$1 hits  in CORMORINO. 
To misidentify a crossing  $\mu$ as a $\chi$ it is necessary that  both hits in the veto counter are missed and only one CORMORINO bar records the hit.
Assuming the veto counter  inefficiency  to be (1-$\epsilon_{veto}$)=5$\%$  and  considering that $\alpha_{Single\; hit}^{Crossing \; \mu}$=32$\%$ for a 1 MeV threshold (36$\%$ for a 10 MeV threshold) of crossing muons release a visible energy in a single CORMORINO bar  (the rejection condition is N$_{Hits}^{Veto}$+N$_{Hits}^{CORMORINO}\ge$2), we end up with a rate of misidentified charged muons of:
\be
R_{Bg}^{Crossing \; \mu} = R^{All\;\mu}\; \alpha_{Single\; hit}^{Crossing \; \mu} \; (1-\epsilon_{veto})^2= 3.3\;10^{-3} {\rm Hz}  \;(3.5\; \;10^{-3} {\rm Hz} )
\ee
\subparagraph{Muons decaying inside CORMORINO}
Muons stopping inside the detector cross one side of the veto.   Positive muons stopping and decaying (at rest)  
 are  all detected for both  thresholds with rate R$^{\mu^+\;inside\;dec}\sim$ 0.12 Hz for  $\mu^+$. 
Negative muons, mainly captured by nuclei,  produce a visible signal in the detector  with rate R$^{\mu^-\;inside\;capture}\sim$ 0.12 Hz  for $\mu^-$   for both thresholds (1 MeV and 10 MeV).\\
Negative muons, if detected by the veto can be rejected. If not detected, and providing a single hit in CORMORINO, they contribute to the background. From MC simulations we derived  $\alpha_{Single\; hit}^{\mu\;inside\;capture}$=24$\%$ for 1 MeV threshold and 39$\%$ for 10 MeV.
\be
R_{Bg}^{\mu^+\ \;inside \; capture} = R^{\mu^-\;inside\;capture}\; \alpha_{Single\; hit}^{\mu\;inside\;capture}\; (1-\epsilon_{veto}) =  1.4\; 10^{-3} {\rm Hz}\;\; (2.4\; 10^{-3} {\rm Hz} )
\ee
Positive muons that release an energy above the trigger threshold (a fraction of R$^{\mu^+\;inside\;dec}$) will provide  a prompt signal (in coincidence with the veto) and a delayed hit due to the positron from $\mu^+ \to e^+ \bar\nu_\mu \nu_e$ . These events can be identified and rejected disregarding hits in the detector during a time window of 10 $\tau_{Decay}=22 \mu$s after the prompt signal. This selection would  add  a negligible dead-time to the DAQ.
A source of background still arises from the veto inefficiency and the fraction of these events that provides a single hit (over threshold) in CORMORINO.
The resulting rate is:
\be
R_{Bg}^{\mu^- \;inside \; decay} = 2\; R^{\mu^-\;inside\;dec}\; \alpha_{Single\; hit}^{\mu\;inside\;dec}\; (1-\epsilon_{veto}) = 2.9\; 10^{-3}{\rm Hz} \;\; (4.8 \; 10^{-3} {\rm Hz} )
\ee
where the factor of 2 takes into account that the stopping muon and/or the positron can both trigger the detector (being $\alpha_{Single\; hit}^{\mu\;inside\;dec}=\alpha_{Single\; hit}^{\mu\;inside\;capture}$).

\subparagraph{Muons decaying inside lead shielding}
Here we consider muons that decay or get captured in the lead shielding between the veto and CORMORINO. We obtained a rate of  
R$^{\mu\;lead}\sim$ 0.9 Hz reduced to 0.3 Hz and 0.2 Hz for a detection  threshold of 1 MeV and 10 MeV respectively.
The fraction of events that deposited energy in a single CORMORINO bar 
%  : is, non are
is $ \alpha_{Single\; hit}^{\mu\;lead}\sim$0.46 and 0.43 for  a threshold of 1 MeV and 10 MeV respectively.
These values lead to a background rate of:
\be
R_{Bg}^{\mu^- \;lead} = R^{\mu\;lead}\; \alpha_{Single\; hit}^{\mu\;lead}\; (1-\epsilon_{veto}) = 7.0\; 10^{-3} {\rm Hz} \;\; (4.3 \; 10^{-3} {\rm Hz} )
\ee

\subparagraph{Muons decaying between iron shielding and  veto}
The last possibility is that the muon decays in the region between the shielding and the veto, mainly  in the very last layer of iron. 
The rate  R$^{\mu\;between\;dec}\sim$ 0.7 Hz. This rate has been estimated considering  the fraction of $\mu$ decaying in the last 10cm of iron all around the detector  corresponding to few absorption lenghts of 20-50 MeV gammas.
For the usual decay, the few  $e^+$ escaping the iron have a good chance to be  detected by the veto and fully absorbed by the lead shielding between the veto and CORMORINO and therefore their contribution to the background is negligible.
The rare  $\mu \to e^- \bar\nu_\mu \nu_e \gamma$ decay  (BR$\sim 1.5 \%$) produces a 20-50 MeV gamma that can enter in CORMORINO bypassing the veto. The absorption length for 10 MeV - 100 MeV gammas in lead is a.l.$\sim$0.9cm.  The leads shielding between the detector and the veto is   5 cm thick, corresponding  to 5.5 a.l. for an overall attenuation of $\sim$~4~10$^{-3}$.  The fraction of  10-100 MeV photon  interacting with CORMORINO and releasing an energy over threshold is estimated to be: $ \alpha_{Single\; hit}^{\mu\;between\;dec}\sim$0.5 for a 1 MeV threshold and 0.2 at 10 MeV. Considering all these factor the background rate is given by:
\be
R_{Bg}^{\mu;\ rare\;dec} = R^{\mu\;between \;dec}\; BR\; Att \; \alpha_{Single\; hit}^{\mu\;between\;dec} = 2\; 10^{-5} {\rm Hz} \; \;(0.8\; 10^{-5}  {\rm Hz} )
\ee
and is therefore negligible.

\begin{table}[htp]
\caption{Expected rates for signal,  beam-related and beam-related background in CORMORINO detector for two detection thresholds: 1 MeV and 10 MeV.}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
 & Rate$_{\;Thr=1 {\rm MeV}}$ (Hz/$\mu{\rm A}$))&Rate$_{\;Thr=10 {\rm MeV}}$ (Hz/$\mu {\rm A}$))\\ 
\hline\hline
 $\chi$ detection  - S.I  & 1.0 10$^{-5}$& 1.2 10$^{-6}$\\
 \hline
$\chi$ detection - S.II  & 2.0 10$^{-7}$ & 0.7 10$^{-7}$\\
 \hline\
B-rel $\nu$ & 2.0 10$^{-9}$ & 2.0 10$^{-10}$\\
 \hline
B-rel neutron  & 0  & 0\\
\hline\hline\hline
 & Rate$_{\;Thr=1 {\rm MeV}}$ (Hz)&Rate$_{\;Thr=10 {\rm MeV}}$ (Hz)\\
\hline\hline
B-unrel $\nu$  &2.0 10$^{-6}$ & 2.0 10$^{-7}$\\
\hline
B-unrel neutron  &2.7 10$^{-3}$ &0.6 10$^{-3}$\\
\hline
Crossing muons  &3.3 10$^{-3}$ &3.5 10$^{-3}$\\
\hline
Captured  $\mu^+$  &1.4 10$^{-3}$  &2.4 10$^{-3}$\\
\hline
Decaying $\mu^-$ (CORM)  &2.9 10$^{-3}$  &4.8 10$^{-3}$\\
\hline
Stopped $\mu$ in lead  &7.0 10$^{-3}$  &4.3 10$^{-3}$\\
\hline
$\mu^-$ rare decay &2.0 10$^{-5}$  &8.0 10$^{-6}$\\
\hline\hline
Total Beam-unrelated bg &1.7 10$^{-2}$  &1.5 10$^{-2}$\\
\hline\hline
\end{tabular}
\end{center}
\label{tab:rates}
\end{table}%

\subsubsection{Summary} 
Rates for  signal,   beam-related and beam-unrelated background sources are reported in Tab.~\ref{tab:rates} for the two detection thresholds of 1 MeV and 10 MeV. 
Based on these estimates we can conclude that beam-related backgrounds are negligible with respect to cosmogenic ones  that represent the dominant source.
This leads  to the consideration  a test-run in this experimental set up would not give us relevant information because of the limited luminosity.
On the other hand, these call for a thorough investigation of beam-unrelated background with a measurement campaign using CORMORINO.
The rates in the table will be  used in the next section to provide an estimate of the   sensitivity for a full scale experiment, with 1 m$^3$ detector in a 6 months rut at 100$\mu$A.


